Learning to Jump from Pixels

Today's robotic quadruped systems can robustly walk over a diverse range of rough but continuous terrains, where the terrain elevation varies gradually. Locomotion on discontinuous terrains, such as those with gaps or obstacles, presents a complementary set of challenges. In discontinuous settings, it becomes necessary to plan ahead using visual inputs and to execute agile behaviors beyond robust walking, such as jumps. Such dynamic motion results in significant motion of onboard sensors, which introduces a new set of challenges for real-time visual processing. The requirement for agility and terrain awareness in this setting reinforces the need for robust control. We present Depth-based Impulse Control (DIC), a method for synthesizing highly agile visually-guided locomotion behaviors. DIC affords the flexibility of model-free learning but regularizes behavior through explicit model-based optimization of ground reaction forces. We evaluate the proposed method both in simulation and in the real world.

==> bc_table.tex <==
\begin{table}[!t]

\centering
\def\arraystretch{1.2}%

\caption{Forward progress across 7.0-meter gapped terrain for RL policies (with Trotting (T), Pronking (P), or Variable-Timing Pronking (VP)) trained on various maximum gap widths with with height maps, depth images as input respectively, and the policy produced by behavioral cloning with and without recurrent architecture. For model trained with maximum gap width $W_{\text{max}}$, the evaluation terrain includes three gaps of width $W_{\text{max}}-5$.} % 
\label{tab:bc_results}

\begin{tabular}{@{}llllll@{}}
\hline
                       Input  & {T, 10cm} & {T, 20cm} & {P, 20cm} & {P, 30cm} & {VP, 30cm} \\ 

Heightmap & 7.0 & 7.0 & 7.0 & 5.5 & 7.0 \\
                % \hline
Depth Image & 5.0 & 3.7 &  & 6.5 & 5.0 \\
                % \hline
BC & 7.0 & 7.0 & 3.3 & 1.9 & 0.8 \\
                % \hline
BC + RNN & 7.0 & 7.0 & 7.0 & 3.3 & 7.0 \\
\hline
\end{tabular}%}




\end{table}

==> ft.tex <==
\begin{figure}[!t]
\begin{subfigure}[b]{0.4\textwidth}
% \vspace{-\topskip}
\centering
\includegraphics[width=0.99\linewidth]{figures/limits.pdf}
\caption{}
\label{fig:performance}
\end{subfigure}
\begin{subfigure}[b]{0.59\textwidth}
% \vspace{-\topskip}
\centering
\def\arraystretch{1.2}%
\resizebox{\columnwidth}{!}{

\begin{tabular}{@{}lllll@{}}
\hline
                       \textit{Width}  & \textit{Heightmap}     & \textit{Depth Image}   & \textit{BC} & \textit{BC + RNN}     \\ \hline

{T, 10cm} & 1.0 (\textit{2}) & 0.59 (\textit{9}) & 0.45  & 0.97 \\
                % \hline
{T, 20cm} & 1.0 (\textit{7}) & 0.18 () & 0.10  & 0.81 \\
                % \hline
{P, 20cm} & 1.0 (\textit{3}) & 0.83 () & 0.05 & 0.91  \\
                % \hline
{P, 30cm} & 1.0 (\textit{8}) & 1.43 (\textit{6}) & 0.03  & 0.17 \\
                % \hline
{VP, 30cm}          & 1.0  & 0.33 &  &  \\ %\hline
{VP, 40cm}          & 1.0 (\textit{2}) & 0.92 (\textit{3}) &  &  \\ \hline
\end{tabular}}

\caption{}
\label{tab:bc_results}
\end{subfigure}%


\caption{\textbf{(a)}:Performance comparison for blind and visually guided policies. Ideal performance is derived from the maximum stride length given velocity and contact schedule constraints. Note that while the theoretical limits are derived assuming zero yaw, the learned trotting controller beats the theoretical limit by assuming nonzero yaw, thus extending the foot placements further apart.
\textbf{(b)}: Normalized episodic reward for RL policies (Trotting (T), Pronking (P), Gait-Free (GF)) trained on various maximum gap widths with with height maps, depth images as input respectively, and the policy produced by behavioral cloning with and without recurrent architecture. For each task, we normalize by the return of the policy trained on heightmaps. Values in parentheses indicate millions of training samples to 90\% convergence for RL. BC performance is reported after 1M training steps. } 

\end{figure}

==> robustness_eval.tex <==
\begin{figure}[!htb]

\begin{subfigure}{0.99\linewidth}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/trot_robustness0.pdf}
    \includegraphics[width=0.32\textwidth]{figures/trot_robustness5.pdf}
    \includegraphics[width=0.32\textwidth]{figures/trot_robustness10.pdf}
    \caption{Robustness of trotting under force perturbation.}
    \label{fig:generalizationtrot}
\end{subfigure}
\hfill
\begin{subfigure}{0.99\linewidth}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/pronk_robustness0.pdf}
    \includegraphics[width=0.32\textwidth]{figures/pronk_robustness10.pdf}
    \includegraphics[width=0.32\textwidth]{figures/pronk_robustness20.pdf}
    \caption{Robustness of pronking under force perturbation.}
    \label{fig:generalizationpronk}
\end{subfigure}
\caption{Performance of trotting and pronking policies under external force perturbation to the base. Perturbations are applied for a duration of 0.3s at random timings, with the average time between perturbations being one second. The bold line represents the mean of $N$ trials; the shaded region represents the interquartile range. }

\label{fig:generalization}
\end{figure}
